Temporal-Rate Encoding to Realize Unary Positional Representation in Spiking Neural Systems

Unary representation is straightforward, error tolerant and requires simple logic while its latency is a concern. On the other hand, positional representation (like binary) is compact and requires less space, but it is sensitive to errors. A hybrid representation called unary positional encoding reduces the latency of unary computation and length of the encoded stream, thus achieves the compactness of positional representation while preserving the error tolerance of unary encoding. In this paper, we discuss the prospect of unary positional encoding in spiking neural systems by incorporating temporal and rate encoding.

==> related.tex <==

The stochastic computing~\cite{stochastic_1969} is based random bit streams that represent the data. The arithmetic operations can be realized with very simple logic, but due to the data representation, the computation takes a long time and data may have a poor precision.
Furthermore, the results are subject to some degree of error due to random
fluctuations. The randomization necessary for data representation can generated by non-trivial circuits that consume area and power.


%In the paradigm of stochastic computing, digital logic is used to perform computation on random bit streams, where input data is represented by the probability.
